Real-Time Word-Level Temporal Segmentation in Streaming Speech Recognition

Rich-text captions are essential to help communication for Deaf and hard-of-hearing (DHH) people, second-language learners, and those with autism spectrum disorder (ASD). They also preserve nuances when converting speech to text, enhancing the realism of presentation scripts and conversation or speech logs. However, current real-time captioning systems lack the capability to alter text attributes (ex. capitalization, sizes, and fonts) at the word level, hindering the accurate conveyance of speaker intent that is expressed in the tones or intonations of the speech. For example, ''YOU should do this'' tends to be considered as indicating ''You'' as the focus of the sentence, whereas ''You should do THIS'' tends to be ''This'' as the focus. This paper proposes a solution that changes the text decorations at the word level in real time. As a prototype, we developed an application that adjusts word size based on the loudness of each spoken word. Feedback from users implies that this system helped to convey the speaker's intent, offering a more engaging and accessible captioning experience.

==> 03_formative_study.tex <==
\section{Formative Study}

==> 04_design.tex <==
\section{Design}


==> 05_implementation.tex <==
\section{Implementation}



==> 06_evaluation.tex <==
\section{Evaluation}

==> 08_conclusion.tex <==
\section{Conclusion}

==> 99_recycle.tex <==
\section{sample code}
\label{sec:sample_section}

inline hogehoge
\xx

inline sentence hogehoge
\xxx

anthony suggestion
\xac


% label, filename, width, caption
when you wanna place wide pictures (See \fgref{samplewidepic})
\textbackslash fgw\{label\}\{filename\}\{width ratio\}\{caption\}
\fgw{samplewidepic}{samplewidepic}{0.8}{\textbackslash fgw\{label (\eg fg:\#1)\}\{filename (\eg figures\slash \{\#2\}.pdf, .jpg,,)\}\{ratio (\eg \{\#3\}\textbackslash textwidth)\}\{caption text (\eg \#4)\}} 

% label, filename, width, caption
when you wanna place pictures according to latex compiler. no specification on the position.(See \fgref{samplefig})
\textbackslash fg\{label\}\{filename\}\{width ratio\}\{caption\}
\fg{samplefig}{samplefig}{0.4}{\textbackslash fg\{label (\eg fg:\#1)\}\{filename (\eg figures\slash \{\#2\}.pdf, .jpg,,)\}\{ratio (\eg \{\#3\}\textbackslash textwidth)\}\{caption text (\eg \#4)\}}

% label, filename, width, caption
when you wanna place pictures like ``HERE!'' (See \fgref{samplegraph})
\textbackslash fgh\{label\}\{filename\}\{width ratio\}\{caption\}
\fgh{samplegraph}{samplegraph}{0.4}{\textbackslash fg\{label (\eg fg:\#1)\}\{filename (\eg figures\slash \{\#2\}.pdf, .jpg,,)\}\{ratio (\eg \{\#3\}\textbackslash textwidth)\}\{caption text (\eg \#4)\}}



Figure hoge
\slash fgref\{\} (like \fgref{samplegraph})

Table hoge
\slash tbref\{\} (like \tbref{sampletable})

Section hoge 
\slash secref\{\} (like \secref{sample_section})


\sssec{how to use subsubsection}
when you want to use subsubsection,
use \textbackslash sssc\{\}. this modified the vspace already.


citation ->
\textbackslash citeref\{Abril07, Cohen07\}. \citeref{Abril07, Cohen07}

\textbackslash eg, \textbackslash ie, \textbackslash etal, \textbackslash vs ->
\eg, \ie, \etal, \vs

\textbackslash one, \textbackslash two, \textbackslash three, \textbackslash four ->
\one \two \three \four

\textbackslash ay, \textbackslash bee, \textbackslash cee, \textbackslash dee ->
\ay \bee \cee \dee


if you want to add some italic bold to cite quotes or something
\textbackslash insec\{poop\} -> \insec{poop}

\textbackslash degree ->
\degree

\td{\textbackslash td to emphasize todo tasks}

\tdfg{\textbackslash tdfg to temporarily pad the figure area}









%%%% sample table
\begin{table}[]
\arraystretch
\caption{Make sure put out an article `a' or `the' from the head of caption sentences.}
\label{tb:sampletable}
\centering
\begin{tabular}{llllll}
\hline
\textbf{what} &
  \textbf{\begin{tabular}[c]{@{}l@{}} Q1 \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}} Q2 \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}} Q3 \end{tabular}} & 
  \textbf{\begin{tabular}[c]{@{}l@{}} Q4 \end{tabular}} &
  \textbf{\xxx} \\ \hline
A &
  \xx &
  \xxx &
  No &
  Yes &
  No \\
B &
  \xx &
  \xxx &
  Yes &
  No &
  Yes \\ \hline
\end{tabular}
\end{table}

==> alt-text.tex <==
Figure 1: \Description[System Workflow and application examples.]{System Workflow and application examples. A) Our system temporally segments streaming Audio Speech Recognition (ASR) results in real time at word level. Workflow in detail is explained in Section.  B) Our system can be used to add word-level nonverbal information (e.g., volume, tones, and intonations) to texts such as those used for subtitles (upper), and to help communicate with people who find it hard to understand the nuances or people who are communicating via translated texts (middle and lower).}
